Game Theory Models for the Verification of the Collective Behaviour of Autonomous Cars

The collective of autonomous cars is expected to generate almost optimal traffic. In this position paper we discuss the multi-agent models and the verification results of the collective behaviour of autonomous cars. We argue that non-cooperative autonomous adaptation cannot guarantee optimal behaviour. The conjecture is that intention aware adaptation with a constraint on simultaneous decision making has the potential to avoid unwanted behaviour. The online routing game model is expected to be the basis to formally prove this conjecture.

==> eptcsdata.tex <==
\providecommand{\firstpage}{27}
\providecommand{\publicationstatus}{L. Bulwahn, M. Kamali, S. Linker (Eds.): First Workshop on\\ Formal Verification of Autonomous Vehicles (FVAV 2017).\\
EPTCS 257, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.257.4}{10.4204/EPTCS.257.4}}

